A Cognitive Radio Based Internet Access Framework for Disaster Response Network Deployment

In this paper, we propose a cognitive radio based Internet access framework for disaster response network deployment in challenged environments. The proposed architectural framework is designed to help the existent but partially damaged networks to restore their connectivity and to connect them to the global Internet. This architectural framework provides the basis to develop algorithms and protocols for the future cognitive radio network deployments in challenged environments.

==> 2_netcod_model.tex <==
%\if@draftclsmode% draft mode uses larger than normal spacing
\def\baselinestretch{1.5} % controls line spacing for draft version
%\fi

\section{Network coding model}
\label{sec:netcod}
We consider ...



==> 3_fairmix.tex <==

%\if@draftclsmode% draft mode uses larger than normal spacing
\def\baselinestretch{1.5} % controls line spacing for draft version
%\fi

\section{Mitigating unfairness in Network Coding}
\label{sec:fairmix}

%\begin{itemize}
%\item Describe FairMix's properties here
%\item put figure with example
%\end{itemize}
\subsection{FairMix Overview}
One solution to alleviate the unfairness in decoding delay of inter-session netwdecoding}


==> 4_perf_ext.tex <==
\section{Performance Analysis}
\label{sec:perf}

This section describes the experiments we have conducted to assess the performan


==> 5_conc.tex <==
\section{Summary and Future Directions}
\label{sec:conc}

Network coding may 

